Optimal Topology Design for Disturbance Minimization in Power Grids

The transient response of power grids to external disturbances influences their stable operation. This paper studies the effect of topology in linear time-invariant dynamics of different power grids. For a variety of objective functions, a unified framework based on $H_2$ norm is presented to analyze the robustness to ambient fluctuations. Such objectives include loss reduction, weighted consensus of phase angle deviations, oscillations in nodal frequency, and other graphical metrics. The framework is then used to study the problem of optimal topology design for robust control goals of different grids. For radial grids, the problem is shown as equivalent to the hard "optimum communication spanning tree" problem in graph theory and a combinatorial topology construction is presented with bounded approximation gap. Extended to loopy (meshed) grids, a greedy topology design algorithm is discussed. The performance of the topology design algorithms under multiple control objectives are presented on both loopy and radial test grids. Overall, this paper analyzes topology design algorithms on a broad class of control problems in power grid by exploring their combinatorial and graphical properties.

==> Properties.tex <==
\section{Optimal Topology Reconfiguration Problem}
\label{sec:properties}
The objective of the ISO, as discussed in the previous section, is to minimize the squared ${\cal H}_2$-norm of the dynamic swing equations. The ${\cal H}_2$ norm of a standard LTI system can be described by the following set of equations \cite{boyd1994linear}: 
\vspace{-0.2cm}
\begin{align} 
||H||^2_{{\cal H}_2} &= \text{Tr}(B^TQB)\label{observability1}\\
A^TQ+QA &= -C^TC \label{observability}
\end{align}
where ($A,B,C$) for our system are the matrices $\begin{bmatrix} 0 &I\\ -M^{-1}L_b  & -M^{-1}D \end{bmatrix}$, $\begin{bmatrix} 0\\ M^{-1}\end{bmatrix}$ and $\begin{bmatrix}L_w^{1/2}  ~&0 \\0 ~&S^{1/2}\end{bmatrix}$, respectively. Matrix $Q = \begin{bmatrix} Q_1 &Q_0\\ Q_0^*  & Q_2\end{bmatrix}$ is positive semi-definite and represents the observability Gramian of the system. As $M$ is a diagonal matrix in our case, the ${\cal H}_2$ norm reduces to 
\begin{align}
||H||^2_{{\cal H}_2} & = \text{Tr}(M^{-1}Q_2M^{-1}) = \text{Tr}(M^{-2}Q_2)\label{H_2eq}
\end{align}
Eq.~(\ref{observability}) can be expanded to:
\begin{subequations}
\footnotesize
\begin{align}
&\begin{bmatrix} 0 &-L_bM^{-1}\\\mathbb{I}   & -DM^{-1} \end{bmatrix}\begin{bmatrix} Q_1 &Q_0\\ Q_0^*  & Q_2\end{bmatrix} +\nonumber\\ &\begin{bmatrix} Q_1 &Q_0\\ Q_0^*  & Q_2\end{bmatrix}\begin{bmatrix} 0 &\mathbb{I}\\ -M^{-1}L_b  & -M^{-1}D \end{bmatrix} =- \begin{bmatrix}L_w  ~&0 \\0 ~&S\end{bmatrix} \label{equalities}
\end{align}
\end{subequations}
This gives us four equality relations, one for each submatrix. The first equality is:
\begin{subequations}
\footnotesize
\begin{align}
&L_b M^{-1}Q_0^*+ Q_0M^{-1}L_b = L_w\\
\Rightarrow~&\text{Tr}((M^{-1}Q_0^*+ Q_0M^{-1})L_bL_b^{+}) = \text{Tr}(L_wL_b^+)\label{cyclic_trace}\\
\Rightarrow~&\text{Tr}((M^{-1}Q_0^*+ Q_0M^{-1})(\mathbb{I} - \frac{11^T}{N}) = \text{Tr}(L_wL_b^+)\label{propertyQ_0}\\
\Rightarrow~&2\text{Tr}(Q_0M^{-1})= \text{Tr}(L_wL_b^+)\label{first_equality}
\end{align}
\end{subequations}
Here, Eq.~(\ref{cyclic_trace}) follows from multiplying both sides by $L_b^+$ (pseudo-inverse of $L_b$), taking trace and then applying the cyclic property of trace. Eq.~(\ref{propertyQ_0}) follows from $L_bL_b^{+} =\mathbb{I} - 11^T/N$, a property of Laplacian matrices \cite{arpita}. Finally, Eq.~(\ref{first_equality}) follows from the property of observability Gramian, $Q_01^T = 0$ \cite{florian}. Multiplying $M^{-1}$ on both sides of the fourth equality from Eq.~(\ref{equalities}), we have 

\begin{subequations}
{\footnotesize
\begin{align}
&D(M^{-1}Q_2+ Q_2M^{-1}D)M^{-1}-(Q_0+ Q_0^*)M^{-1} = SM^{-1}\nonumber\\
&\Rightarrow~ 2d\text{Tr}(M^{-2}Q_2) = 2\text{Tr}(Q_0M^{-1}) + \text{Tr}(SM^{-1})\label{second_equality}\\
&\Rightarrow~ \text{Tr}(M^{-2}Q_2) = (\text{Tr}(L_wL_b^+) + \text{Tr}(SM^{-1}))/2d \label{combine}
\end{align}}
\end{subequations}
Here, Eq.~(\ref{second_equality}) follows from the cyclic property of trace and Assumption $1$ where $D = d\mathbb{I}$. Finally, Eq.~(\ref{combine}) follows from Eq.~(\ref{first_equality}). Eqs.~(\ref{H_2eq},\ref{combine}) thus give us a closed form of the squared ${\cal H}_2$ norm of the system that is summarized in the following lemma.
\begin{lem}\label{H_2lemma}
The squared ${\cal H}_2$ norm of the LTI dynamical system given by Eqs.~(\ref{swingmatrixfull},\ref{output}) is given by $(\text{Tr}(L_wL_b^+) + \text{Tr}(SM^{-1}))/2d$.
\end{lem}
Without Assumption $1$ (constant damping), Eq.~(\ref{combine}) will provide a bound on the squared ${\cal H}_2$ norm based on the maximum and minimum values of nodal damping. A similar albeit restricted formulation with additionally fixed nodal inertia is derived in \cite{gayme} where Laplacian matrices $L_w$ and $L_b$ are defined over the same grid graph.

Note that in Lemma \ref{H_2lemma}, the effect of $S$ (weights associated with frequency deviations) on the ${\cal H}_2$ norm is separable from that of the grid topology (or $L_b$). Thus, the search for the optimal grid topology can be limited to the first term of Lemma \ref{H_2lemma}. This provides the following reformulation of Problem \ref{problem}:
\begin{subequations}
\begin{align}
    \argmin_{{\cal E} \in {\cal E}^{full}} ~&\text{Tr}(L_wL_b^+)\\
     \text{s.t.}~ & |{\cal E}| = k, \  rank(L_b) = N-1 \label{rank}
\end{align}
\label{problem_1}
\end{subequations}
The $N-1$ rank constraint for $L_b$ ensures that the graph constructed using set $\cal E$ has one connected component. Note that brute force schemes to determine the optimal topology quickly become intractable due to the exponential number of candidate feasible graphs that can be constructed.

\subsection{Pseudo-inverse and graph distances}
We now use properties of Laplacian pseudo-inverse to describe Problem \ref{problem_1} in terms of effective graph distances. This will enable us to relate Problem \ref{problem_1} to studied problems in graph theory. By definition, $L_b^+(i,i)+ L_b^+(j,j) - 2L_b^+(i,j)$ is termed the effective susceptance ($b_{eff}(i,j)$) between nodes $i$ and $j$ in the graph. Effective susceptance (similar to effective resistance) represents the effective ratio between voltage difference between nodes $i$ and $j$ when one unit of current is inserted at $i$ and taken out at $j$. We can expand the optimization function in Problem \ref{problem_1} as follows: 

\begin{subequations}
{\footnotesize
\begin{align}
\text{Tr}(L_wL_b^+) &= \sum_{\forall i \neq j}w_{ij}(L_b^+(i,i)+ L_b^+(j,j) - 2L_b^+(i,j))\label{graph_eq1}\\
&= \sum_{\forall i \neq j}w_{ij}b_{eff}(i,j) \label{graph_eq}
\end{align}}
\end{subequations}
Note that for $i \neq j$,  $L_w(i,j) = -w_{ij}$. On the other hand, the effective susceptance $b_{eff}(i,j)$ concerns edges that arise from the Laplacian matrix $L_b$. The optimal topology design problem \ref{problem_1} can now interpreted as:
\begin{lem}\label{graph_distance}
The optimization function in Problem \ref{problem_1} is equivalent to \textit{minimizing the weighted sum of effective susceptances between all nodes pairs in the graph}.  
\end{lem}
The expression in Eq.~(\ref{graph_eq}) can also be listed in terms of the \textit{reduced} Laplacian matrices $\hat{L}_w, \hat{L}_b$ of size $(N-1)\times (N-1)$. Note that the reduction is achieved by deleting the row and column corresponding to a fixed reference node $r$ from $L_w$ and $L_b$ respectively. This is commonly done in power system analysis as reduced Laplacians of connected graphs have full rank. It is well known that the inverse of $\hat{L}_b$ and the pseudo-inverse ($L_b^+$) of $L_b$ are related by the following equation \cite{arpita}: 
$$\hat{L}^{-1}_b(i,j) = (L_b^+(i,j) -L_b^+(i,r)) - (L_b^+(r,j) -L_b^+(r,r))$$
Using this with Eq.~(\ref{graph_eq1}), the following result follows immediately:
\begin{lem} \label{laplacian_commute}
For weighted Laplacian matrices $L_w$ and $L_b$ defined over two connected graphs over the same set of nodes, $\text{Tr}(L_wL_b^+)= \text{Tr}(\hat{L}_w\hat{L}^{-1}_b)$.
\end{lem}
Note that the two Laplacian matrices $L_w$ and $L_b$ need not correspond to the same set of edges. This result generalizes a similar result in \cite{gayme} where $L_w$ and $L_b$ are restricted to include the same edges. In Section \ref{sec:meshnetwork}, we use Lemma \ref{laplacian_commute} to prove an useful supermodular property. In the next two sections, we analyze two variants of the optimal topology design  problem: one for radial networks and the other for meshed networks. In particular, we discuss their computational hardness and solution schemes.








